An Inexact Semi-smooth Newton Method on Riemannian Manifolds with Application to Duality-based Total Variation Denoising

We propose a higher-order method for solving non-smooth optimization problems on manifolds. In order to obtain superlinear convergence, we apply a Riemannian Semi-smooth Newton method to a non-smooth non-linear primal-dual optimality system based on a recent extension of Fenchel duality theory to Riemannian manifolds. We also propose an inexact version of the Riemannian Semi-smooth Newton method and prove conditions for local linear and superlinear convergence that hold independent of the sign of the curvature. Numerical experiments on l2-TV-like problems with dual regularization confirm superlinear convergence on manifolds with positive and negative curvature.

==> asytmp/ex_article-1+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1+0_0}%
}%


==> asytmp/ex_article-1.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 47.147050pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,23.573525)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-1+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-1,3Daac=13.3645134,3Dc2w=-0.995383407 0 -0.095978503 0 1 0 0.095978503 0 -0.995383407 73.513795295 0.442838323 198.693052334,3Droo=200.068685977,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-1+0_0.pdf}}}{\ASYprefix\jobname-1+0.prc}}%


==> asytmp/ex_article-10+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-10+0_0}%
}%


==> asytmp/ex_article-10.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 187.671700pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,93.835850)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-10+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-10,3Daac=37.869871228,3Dc2w=-0.999916561 0 0.012917824 -0.000999789 0.997000427 -0.077389598 -0.012879076 -0.077396056 -0.996917238 76.936767288 91.466243422 272.446885092,3Droo=267.712086988,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-10+0_0.pdf}}}{\ASYprefix\jobname-10+0.prc}}%


==> asytmp/ex_article-11+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-11+0_0}%
}%


==> asytmp/ex_article-11.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 206.762990pt{}%
\kern 203.731670pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.865835,103.381495)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-11+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-11,3Daac=39.891321042,3Dc2w=-0.999939661 0 -0.01098519 0.000200987 0.999832611 -0.018295059 0.010983351 -0.018296163 -0.999772282 81.974661107 85.876030742 279.127700255,3Droo=279.213907238,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-11+0_0.pdf}}}{\ASYprefix\jobname-11+0.prc}}%


==> asytmp/ex_article-12+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-12+0_0}%
}%


==> asytmp/ex_article-12.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 202.727930pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,101.363965)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-12+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-12,3Daac=39.37558292,3Dc2w=-0.999958229 0 -0.00914004 0.000024153 0.999996509 -0.002642398 0.009140008 -0.002642508 -0.999954738 87.368455174 88.752832397 277.073173324,3Droo=277.091841512,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-12+0_0.pdf}}}{\ASYprefix\jobname-12+0.prc}}%


==> asytmp/ex_article-13+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-13+0_0}%
}%


==> asytmp/ex_article-13.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 203.751750pt{}%
\kern 203.731670pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.865835,101.875875)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-13+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=None,3Dmenu,3Dtoolbar=false,label=ex_article-13,3Daac=34.177666386,3Dc2w=0.371390676 -0.928476691 0 -0.169515876 -0.06780635 0.98319208 -0.912870929 -0.365148372 -0.182574186 296.573046165 118.628900385 59.363965781,3Droo=324.88838975,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-13+0_0.pdf}}}{\ASYprefix\jobname-13+0.prc}}%


==> asytmp/ex_article-2+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-2+0_0}%
}%


==> asytmp/ex_article-2.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 23.057120pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,11.528560)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-2+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-2,3Daac=6.810657047,3Dc2w=-0.991547822 0 -0.129741729 0 1 0 0.129741729 0 -0.991547822 65.478619144 0.227007639 194.569644021,3Droo=197.06712375,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-2+0_0.pdf}}}{\ASYprefix\jobname-2+0.prc}}%


==> asytmp/ex_article-3+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-3+0_0}%
}%


==> asytmp/ex_article-3.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 55.177040pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,27.588520)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-3+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-3,3Daac=15.464232997,3Dc2w=-0.999900015 0 0.014140716 0 1 0 -0.014140716 0 -0.999900015 87.977880218 -0.144032262 201.692370113,3Droo=201.721992275,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-3+0_0.pdf}}}{\ASYprefix\jobname-3+0.prc}}%


==> asytmp/ex_article-4+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-4+0_0}%
}%


==> asytmp/ex_article-4.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 23.057120pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,11.528560)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-4+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-4,3Daac=6.810657047,3Dc2w=-0.991547822 0 -0.129741729 0 1 0 0.129741729 0 -0.991547822 65.478619144 0.227007639 194.569644021,3Droo=197.06712375,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-4+0_0.pdf}}}{\ASYprefix\jobname-4+0.prc}}%


==> asytmp/ex_article-5+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-5+0_0}%
}%


==> asytmp/ex_article-5.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 28.075850pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,14.037925)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-5+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-5,3Daac=7.812017807,3Dc2w=-0.999427837 0 0.033823045 0 1 0 -0.033823045 0 -0.999427837 96.015165053 0.433263417 207.946027185,3Droo=208.173703557,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-5+0_0.pdf}}}{\ASYprefix\jobname-5+0.prc}}%


==> asytmp/ex_article-6+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-6+0_0}%
}%


==> asytmp/ex_article-6.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 33.094580pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,16.547290)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-6+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-6,3Daac=9.185644165,3Dc2w=-0.999609359 0 0.027948686 0 1 0 -0.027948686 0 -0.999609359 92.698440293 0.34161721 207.169834683,3Droo=207.310143336,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-6+0_0.pdf}}}{\ASYprefix\jobname-6+0.prc}}%


==> asytmp/ex_article-7+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-7+0_0}%
}%


==> asytmp/ex_article-7.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 33.094580pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,16.547290)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-7+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-7,3Daac=9.159126436,3Dc2w=-0.999609359 0 0.027948686 0 1 0 -0.027948686 0 -0.999609359 92.719723454 0.340741705 207.760893726,3Droo=207.901566325,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-7+0_0.pdf}}}{\ASYprefix\jobname-7+0.prc}}%


==> asytmp/ex_article-8+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-8+0_0}%
}%


==> asytmp/ex_article-8.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 33.094580pt{}%
\kern 203.751750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.875875,16.547290)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-8+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-8,3Daac=9.159126436,3Dc2w=-0.999609359 0 0.027948686 0 1 0 -0.027948686 0 -0.999609359 92.719723454 0.340741705 207.760893726,3Droo=207.901566325,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-8+0_0.pdf}}}{\ASYprefix\jobname-8+0.prc}}%


==> asytmp/ex_article-9+0.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-9+0_0}%
}%


==> asytmp/ex_article-9.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 210.777980pt{}%
\kern 203.731670pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-101.865835,105.388990)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-9+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=ex_article-9,3Daac=39.841398808,3Dc2w=-0.999777369 0 0.021100074 -0.002596198 0.992401445 -0.123014758 -0.020939744 -0.123042151 -0.992180506 87.851209166 110.738759984 281.631770342,3Droo=284.368964037,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-9+0_0.pdf}}}{\ASYprefix\jobname-9+0.prc}}%


==> sections/A-GCov-computation.tex <==
\section{Derivation of the Generalized Covariant Derivative}
\label{app: derive cov}

Next

Actually evaluating the generalized covariant derivative \cref{eq: Newton} for a general manifold can be complicated. However, in the case of symmetric manifolds, this becomes much easier. For symmetric manifolds we know the differentials and/or covariant derivatives of geodesics, exponential and logarithmic maps \cite[Prop ?]{bergmann2018recent} \todo{dit}. If we also use that in symmetric spaces the parallel transport map is exactly the pole ladder \cite{pennec2018parallel} - which is also formulated in terms of logarithmic, exponential and geodesic maps - we have exact expressions for the full generalized covariant derivative, with the exception of the differentials of the proximal maps. As we shall see in the next section, for $\ell^2$-TV we even have exact expressions for the proxes on top of that.
\subsection{The Generalized Covariant Derivative for the Exact Newton System}
Let $\mathcal{M}$ and $\mathcal{N}$ be symmetric manifolds. In the case of the exact optimality conditions \cref{eq: primal eq} and \cref{eq: dual eq} we constructed the vector field $X_e: \mathcal{M} \times \mathcal{T}_{n}^* \mathcal{N} \rightarrow \mathcal{T} \mathcal{M} \times \mathcal{T}_{n}^* \mathcal{N}$ given by
\begin{equation}
	\label{eq: X exact}
	X_e(p,\xi) = \begin{pmatrix}
		- \log_p \operatorname{prox}_{\sigma F}\left(\exp _{p}\left(\mathcal{P}_{m \rightarrow p}\left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} \xi_{n}\right]\right)^{\sharp}\right)\right)\\ 
		\xi_{n} - \operatorname{prox}_{\tau G^*_{n}}\left(\xi_{n}+\tau\left(\log _{n} \Lambda\left(p\right)\right)^{\flat}\right)
	\end{pmatrix}.
\end{equation}
In the following the four components of the operator $V_e \in \mathcal{L}(\mathcal{T}_p \mathcal{M} \times \mathcal{T}_{n}^* \mathcal{N})$ will be constructed so that
\begin{equation}
	V_e =  \begin{bmatrix}
		V_{e,1,p} & V_{e,1,\xi_n} \\ 
		V_{e,2,p} & V_{e,2,\xi_n}
	\end{bmatrix} \in \partial_{\mathcal{M},C} X_e(p,\xi_n).
\end{equation}

\paragraph{Compute $ V_{e,1,p}$}
For $\partial_{\mathcal{M},C,p} X_{e,1}$ we need to compute

\begin{align}
	&\partial_{\mathcal{M},C,p} X_{e,1} = - \partial_{C,p} \log_{(\cdot)} \operatorname{prox}_{\sigma F}\left(\exp _{p}\left(\mathcal{P}_{m \rightarrow p}\left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} \xi_{n}\right]\right)^{\sharp}\right)\right) \nonumber \\
	&-  D_{C,p} \log_p \operatorname{prox}_{\sigma F}\left(\exp _{(\cdot)}\left(\mathcal{P}_{m \rightarrow (\cdot)}\left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} \xi_{n}\right]\right)^{\sharp}\right)\right).
\end{align}
In order to compute the second term, we will use the chain rule. For that we will pass to the the pole ladder
\begin{align}
	P_{m \rightarrow p}^{\mathrm{P}}(\xi) & =-\log _{p}\left(\gamma\left(\exp _{m}(\xi), \gamma\left(m, p ; \frac{1}{2}\right) ; 2\right)\right)\\
	& = -\log _{p} \left(\exp_{\exp _{m}(\xi)}\left(2\log_{\exp _{m}(\xi)} \gamma\left(m, p ; \frac{1}{2}\right)\right)\right)
	\label{eq: pole ladder rewritten}
\end{align}
as substitution for the parallel transport map. Remember that this is exact for symmetric manifolds. If we rewrite the pole ladder as in \cref{eq: pole ladder rewritten} then we get for the differential
\begin{align}
	&\partial_{\mathcal{M},C,p} X_{e,1} = - \partial_{C,p} \log_{(\cdot)} \operatorname{prox}_{\sigma F}\left(\exp _{p}\left(\mathcal{P}_{m \rightarrow p}\left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} \xi_{n}\right]\right)^{\sharp}\right)\right) \nonumber \\
	& -  D_{C,p} \log_p \operatorname{prox}_{\sigma F}\left(\exp _{(\cdot)}\left( -\log _{(\cdot)}\left(\exp_{\exp_{m}(q_\xi(\xi))}\left(2\log_{\exp _{m}(q_\xi(\xi))} \gamma\left(m, (\cdot) ; \frac{1}{2}\right)\right)\right)\right)\right).
\end{align}

Now, let 
\begin{subequations}
	\begin{align}
		q_0(p,\xi)& := \operatorname{prox}_{\sigma F}\left(\exp _{p}\left(\mathcal{P}_{m \rightarrow p}\left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} \xi_{n}\right]\right)^{\sharp}\right)\right), \\
		q_1(p,\xi) &:= \operatorname{prox}_{\sigma F}\left(q_2 (p,\xi)\right), \\
		q_2 (p,\xi) &:= \exp _{p}\left(q_3(p,\xi)\right),\\
		q_3(p,\xi) &:= -\log_p (q_4(p,\xi)),\\
		%&\mathcal{P}_{m \rightarrow p}\left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} \xi_{n}\right]\right)^{\sharp}\\
		q_4(p,\xi) &:= \exp_{\exp_{m}(q_\xi(\xi))} (q_5(p,\xi)),\\
		q_5 (p,\xi) &:= 2\log_{\exp_{m}(q_\xi(\xi))} (q_p(p)),\\
		q_\xi(\xi)  &:= \left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} \xi_{n}\right]\right)^{\sharp},\\
		q_p (p) &:= \gamma\left(m, p ; 1/2\right).
	\end{align}
\end{subequations}
Then 
\begin{align}
	V_{e,1,p} := A_1 + A_2 B \left[ C_1 + C_2\left[D_1 + D_2 E F G \right]\right] \in \partial_{\mathcal{M},C,p} X_{e,1},
\end{align}
where
\begin{subequations}
	\begin{align}
		A_1 & := - \nabla \log_{(\cdot)} q_0(p,\xi)\big|_p,\\
		A_2 & := - D_{q_1(p,\xi)} \log_p (\cdot),\\
		B & \in D_{C,q_2(p,\xi)} \operatorname{prox}_{\sigma F} (\cdot), \\
		C_1 & :=  D_{p} \exp_{(\cdot)} q_3 (p,\xi),\\
		C_2 & :=  D_{q_3 (p,\xi)} \exp_{p} (\cdot),\\
		D_1 & := - (D_p \log_{(\cdot)} q_4 (p,\xi))^v = (\nabla \log_{(\cdot)} q_4 (p,\xi))\big|_p,\\
		D_2 &:=  - D_{q_4 (p,\xi)} \log_{p} (\cdot) ,\\
		E &:= D_{q_5 (p,\xi)} \exp_{\exp_{m}(q_\xi(\xi))} (\cdot),\\
		F &:= 2 D_{q_p (p)} \log_{\exp_{m}(q_\xi(\xi))} (\cdot), \\
		G &:= D_p \gamma\left(m, (\cdot) ; 1/2 \right).
	\end{align}
\end{subequations}
Note that the only non-smoothness can come from the proximal mapping.

\paragraph{Compute $V_{e,1,\xi_n}$}
For $D_{C,\xi_n} X_{e,1}$ we need to compute
\begin{align}
	D_{C,\xi_n} X_{e,1} = -  D_{C,\xi_n} \log_p \operatorname{prox}_{\sigma F}\left(\exp _{p}\left(\mathcal{P}_{m \rightarrow p}\left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} (\cdot)\right]\right)^{\sharp}\right)\right).
\end{align}
Now note that $H:\mathcal{T}^*_n\mathcal{N}\rightarrow \mathcal{T}_p\mathcal{M}$ given by
\begin{equation}
	\xi \mapsto \mathcal{P}_{m \rightarrow p}\left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} \xi \right]\right)^{\sharp}
\end{equation}
is a linear map. Hence the differential will be
\begin{equation}
	V_{e,1,\xi_n} := A_2 B C_2 H \in D_{C,\xi_n} X_{e,1} ,
\end{equation}
where $A_2$, $B$ and $C_2$ as described before.

\paragraph{Compute $V_{e,2,p}$}
For $D_{C,p} X_{e,2}$ we need to compute
\begin{align}
	D_{C,p} X_{e,2} &= D_{p}\xi_{n} - D_{C,p}\operatorname{prox}_{\tau G^*_{n}}\left(\xi_{n}+\tau\left(\log _{n} \Lambda\left(p\right)\right)^{\flat}\right)\\
	& = - D_{C,p}\operatorname{prox}_{\tau G^*_{n}}\left(\xi_{n}+\tau\left(\log _{n} \Lambda\left(p\right)\right)^{\flat}\right).
\end{align}
Let
\begin{subequations}
	\begin{align}
		\tilde{\eta}_1(p,\xi) & := \xi_{n}+\tau\left(\log _{n} \Lambda\left(p\right)\right)^{\flat},\\
		\eta_p(p) & := \Lambda(p).
	\end{align}
\end{subequations}
Then 
\begin{align}
	V_{e,2,p} := - JKLM \in D_{C,p} X_{e,2},
\end{align}
where
\begin{subequations}
	\begin{align}
		J & \in   D_{\eta_1(p,\xi)}\operatorname{prox}_{\tau G^*_{n}} (\cdot), \\
		K &:= \tau \flat,\\
		L & := D_{\eta_p(p)} \log_n (\cdot),\\
		M & :=  D_{p}\Lambda (\cdot).
	\end{align}
\end{subequations}
\todo{Ronny: typo flat}
\paragraph{Compute $V_{e,2,\xi_n}$}
Finally, for $\partial_{C,\xi} X_{e,2}$ we find
\begin{align}
	\partial_{C,\xi_n} X_{e,2} &= I - \partial_{C,\xi_n}\operatorname{prox}_{\tau G^*_{n}}\left(\xi_{n}+\tau\left(\log _{n} \Lambda\left(p\right)\right)^{\flat}\right)\\
	\Rightarrow \quad V_{e,2,\xi_n} := &  I - J \in \partial_{C,\xi_n} X_{e,2},
\end{align}
where $I$ is the identity and $J$ as described in the previous step.

\subsection{The Generalized Covariant Derivative for the Linearized Newton System}
Again let $\mathcal{M}$ and $\mathcal{N}$ be symmetric manifolds. In the case of the linearized optimality conditions \cref{eq: primal eq 2} and \cref{eq: dual eq 2} we constructed the vector field $X_l: \mathcal{M} \times \mathcal{T}_{n}^* \mathcal{N} \rightarrow \mathcal{T} \mathcal{M} \times \mathcal{T}_{n}^* \mathcal{N}$ given by
\begin{equation}
	X_l(p,\xi) = \begin{pmatrix}
		- \log_p \operatorname{prox}_{\sigma F}\left(\exp _{p}\left(\mathcal{P}_{m \rightarrow p}\left(-\sigma(D_m \Lambda)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda(m)} \xi_{n}\right]\right)^{\sharp}\right)\right)\\ 
		\xi_{n} - \operatorname{prox}_{\tau G_{n}^{*}}\left(\xi_{n}+\tau\left(\mathcal{P}_{\Lambda\left(m\right) \rightarrow n} D_m \Lambda\left[\log _{m} p\right]\right)^{\flat}\right)
	\end{pmatrix}.
\end{equation}
For computing the components of the operator $V_l \in \mathcal{L}(\mathcal{T}_p \mathcal{M} \times \mathcal{T}_{n}^* \mathcal{N})$, note that only the dual component has changed compared to \cref{eq: X exact}. Hence step 1 and 2 of the previous part are the same: $V_{l,1,p} = V_{e,1,p}$ and $V_{l,1,\xi_n} = V_{e,1,\xi_n}$. For the derivative $\partial_{C,\xi} X_{l,2}$ we will not get anything different as well: $V_{l,2,\xi_n} = V_{l,2,\xi_n}$. So only $V_{l,2,p}$ will be different.

For $D_{C,p} X_{l,2}$ we need to compute
\begin{align}
	D_{C,p} X_{l,2} &= D_{p}\xi_{n} - D_{C,p}\operatorname{prox}_{\tau G^*_{n}}\operatorname{prox}_{\tau G_{n}^{*}}\left(\xi_{n}+\tau\left(\mathcal{P}_{\Lambda\left(m\right) \rightarrow n} D_m \Lambda\left[\log _{m} p\right]\right)^{\flat}\right)\\
	& = - D_{C,p}\operatorname{prox}_{\tau G_{n}^{*}}\left(\xi_{n}+\tau\left(\mathcal{P}_{\Lambda\left(m\right) \rightarrow n} D_m \Lambda\left[\log _{m} p\right]\right)^{\flat}\right).
\end{align}
Let
\begin{align}
	\tilde{\eta}_1(p,\xi) := \xi_{n}+\tau \mathcal{P}_{\Lambda\left(m\right) \rightarrow n} D_m \Lambda \left[\log _{m} p\right].
\end{align}
Then 
\begin{align}
	V_{l,2,p} := - \tilde{J}K\tilde{L}\tilde{M} \in D_{C,p} X_{l,2} ,
\end{align}
where $K$ as before and
\begin{subequations}
	\begin{align}
		\tilde{J} & \in   D_{\tilde{\eta}_1(p,\xi)}\operatorname{prox}_{\tau G^*_{n}} (\cdot), \\
		\tilde{L} & := \mathcal{P}_{\Lambda\left(m\right) \rightarrow n} D_m \Lambda,\\
		\tilde{M} & :=  D_{p}\log_m (\cdot).
	\end{align}
\end{subequations}


\subsection{Building the Newton Matrix}
In the previous we constructed two linear operators: the generalized covariant derivative for the exact and the linearized optimality system. In practice a matrix is preferable. To construct a matrix representation of an operator 
\begin{equation}
	V = \begin{bmatrix}
		V_{1,p} & V_{1,\xi_n} \\ 
		V_{2,p} & V_{2,\xi_n}
	\end{bmatrix}\in \partial_{C,\mathcal{M}} X(p,\xi_n),
\end{equation}
we will need a basis. Let $\{\Theta_j\}_j$ be an orthonormal basis for $\mathcal{T}_p \mathcal{M}$ and let $\{\Xi_j\}_j$ be a basis for $\mathcal{T}_n^* \mathcal{N}$. Then, we want to find of $U$ and $W$ in this basis, i.e, find $\{u^j\}_j$ and $\{w^j\}_j$ such that
\begin{equation}
	U = \sum_{j = 1}^{M} u^j \Theta_j \quad \text{and} \quad W = \sum_{j = 1}^{N} w^j \Xi_j
\end{equation}
solve the system 
\begin{align}
	&	\sum_{j}^{M} \langle \Theta_i, V_{1,p} [\Theta_j] \rangle u^j + \sum_{j}^{N} \langle \Theta_i, V_{1,\xi} [\Xi_j] \rangle w^j = - \langle \Theta_i, X_1 \rangle  \qquad  i = 1,2,...,M, \\
	& 	\sum_{j}^{M} \langle \Xi_i, V_{2,p} [\Theta_j] \rangle u^j + \sum_{j}^{N} \langle \Xi_i, V_{2,\xi} [\Xi_j] \rangle w^j = - \langle \Xi_i, X_2 \rangle  \qquad  i = 1,2,...,N,
\end{align}
where $M$ is the dimension of $\mathcal{M}$ (and hence also of $\mathcal{T}_p \mathcal{M}$) and $N$ that of $\mathcal{N}$ (and again also that of $\mathcal{T}_n^* \mathcal{N}$). 

==> sections/A-GCov-derivation.tex <==
\section{Derivation of the Generalized Covariant Derivative}
\label{app: cov derivation}
Now that the vector fields 
\begin{equation}
	X_e(p,\xi_n) := \begin{pmatrix}
		-\log_p \operatorname{prox}_{\sigma F}\left(\exp _{p}\left(\mathcal{P}_{m\rightarrow p} \left(-\sigma \left(D_m \Lambda\right)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda\left(m\right)} \xi_{n}\right]\right)^{\sharp}\right)\right)\\ 
		\xi_{n} - \operatorname{prox}_{\tau G^*_{n}}\left(\xi_{n}+\tau\left(\log _{n} \Lambda\left(p\right)\right)^{\flat}\right)
	\end{pmatrix}
\end{equation}
and
\begin{equation}
	X_l(p,\xi_n) := \begin{pmatrix}
		-\log_p \operatorname{prox}_{\sigma F}\left(\exp _{p}\left(\mathcal{P}_{m\rightarrow p} \left(-\sigma \left(D_m \Lambda\right)^{*}\left[\mathcal{P}_{n \rightarrow \Lambda\left(m\right)} \xi_{n}\right]\right)^{\sharp}\right)\right)\\ 
		\xi_{n} - \operatorname{prox}_{\tau G_{n}^{*}}\left(\xi_{n}+\tau\left(\mathcal{P}_{\Lambda\left(m\right) \rightarrow n} D_m \Lambda\left[\log _{m} p\right]\right)^{\flat}\right)
	\end{pmatrix}
\end{equation}
have been constructed, we pass to a general
\begin{equation}
	X(p,\xi_n) := (X_1(p,\xi_n),X_2(p,\xi_n)) := (-\log_p f_1(p,\xi_n), \xi_n - f_2(p,\xi_n)),
\end{equation}
where $f_1: \mathcal{M}\times \mathcal{T}_n^*\mathcal{N}\rightarrow \mathcal{M}$ and $f_2: \mathcal{M}\times \mathcal{T}_n^*\mathcal{N}\rightarrow \mathcal{T}_n^*\mathcal{N}$ are the mappings corresponding to either the exact or the linearized system. In order to proceed with RSSN, the generalized covariant derivative of $X$ must be constructed. 
%To get started, we must first realize that both components of our $X$ are compositions of maps. 
The main idea of finding the Newton operator, both for the exact and the linearized system, follows from rewriting the covariant derivative along $\gamma := (\gamma_1,\gamma_2): (-\epsilon,\epsilon)\rightarrow \mathcal{M}\times \mathcal{T}_n^*\mathcal{N}$ as separate contributions from $\gamma_1:(-\epsilon,\epsilon)\rightarrow \mathcal{M}$ and from $\gamma_2:(-\epsilon,\epsilon)\rightarrow \mathcal{T}_n^*\mathcal{N}$. Let $M$ be the dimension of $\mathcal{M}$ and $N$ the dimension of $\mathcal{T}_n^*\mathcal{N}$. Then, by passing to normal coordinates $(U,\phi)$ on $\mathcal{M}$ and $(V,\psi)$ on $\mathcal{T}_n^*\mathcal{N}$ originating at $(p,\xi_n)$\footnote{Note that we might as well say $(p,0)$ since the second component is a vector space and hence we have $\mathcal{T}_{\xi_n}\mathcal{T}_n^*\mathcal{N} \cong \mathcal{T}_n^*\mathcal{N} $,i.e., we might as well take the origin here.} we can find basis $\{\Theta \}_i^M$ and $\{\Xi\}_j^N$ and coordinates $u_1^{i} \in C^\infty((-\epsilon,\epsilon))$, $ x_1^{i} \in C^\infty((-\epsilon,\epsilon)) $ for $ i = 1,...,M$ and $u_2^{j}\in C^\infty((-\epsilon,\epsilon))$, $x_2^{j} \in C^\infty((-\epsilon,\epsilon)) $ for $ j = 1,...,N$ and write
\begin{equation}
	\gamma_1 = \sum_{i}^M u_1^{i} \Theta_{i} \quad \text{ and }\quad X_1=\sum_{i}^N x_1^{i} \Theta_{i}
\end{equation}
and
\begin{equation}
	\gamma_2 = \sum_{j}^M u_2^{j} \Xi_{j} \quad \text{ and }\quad X_2=\sum_{j}^N x_2^{j} \Xi_{j}.
\end{equation}
If we now first assume that $X$ is smooth. Then, bringing the latter expressions this into the covariant derivative as in \cref{eq: cov deriv} and denoting $\Psi_k \in \{\Theta \}_i^M \cup \{\Xi\}_j^N$ as either basis vector we can write 

\begin{align}
	\frac{D X}{d t}&=\sum_{k}^{M+N}\left(\frac{d x^{k}}{d t}+\sum_{i, j}^{M+N} \Gamma_{i j}^{k} x^{i} u^j\right) \Psi_{k}\\
	&=\sum_{i}^M\left(\frac{d x_1^{k}}{d t}\right) \Theta_{i} + \sum_{j}^N\left(\frac{d x_2^{k}}{d t}\right) \Xi_{j} + \sum_{k}^{M+N}\left(\sum_{i, j}^{M+M} \Gamma_{i j}^{k} x^{i} u^j\right) \Psi_{k} \\
	&=\sum_{i}^M\left(\frac{d x_1^{k}}{d t_1} + \frac{d x_1^{k}}{d t_2}\right) \Theta_{i} + \sum_{j}^N\left(\frac{d x_2^{k}}{d t_1} + \frac{d x_2^{k}}{d t_2}\right) \Xi_{j} + \sum_{k}^{M+N}\left(\sum_{i, j}^{M+M} \Gamma_{i j}^{k} x^{i} u^j\right) \Psi_{k} \\
	& = \frac{D X_1}{d t_1} +\sum_{i}^M\left(\frac{d x_1^{k}}{d t_2}\right) \Theta_{i} + \sum_{j}^N\left(\frac{d x_2^{k}}{d t_1}\right) \Xi_{j}+ \frac{D X_2}{d t_2} + \sum_{k}^{M+N}\left(\sum_{i, j}^{M+M} \Gamma_{i j}^{k} x^{i} u^j\right) \Psi_{k}.
\end{align}
We need the covariant derivative at $t = 0$, i.e., at $(p,\xi_n)$. So let $\eta_p = \dot{\gamma}_1(0)$ and $\eta_\xi = \dot{\gamma}_2(0)$. Also note that $\Gamma_{i j}^{k}\big|_{t=0} = 0$ since we work in normal coordinates. Then
\begin{align}
	\nabla_{\eta_p + \eta_{\xi_n}} X  &= \frac{D X}{d t} \bigg|_{t=0} \\
	&= \frac{D X_1}{d t_1}\bigg|_{t=0} +\sum_{i}^M\left(\frac{d x_1^{k}}{d t_2}\right)\bigg|_{t=0} \Theta_{i} + \sum_{j}^N\left(\frac{d x_2^{k}}{d t_1}\right)\bigg|_{t=0} \Xi_{j}+ \frac{D X_2}{d t_2}\bigg|_{t=0} \\
	& = \frac{D X_1}{d t_1}\bigg|_{t=0} + D_{\xi_n}X_1[\eta_{\xi_n}] + D_{p}X_2[\eta_{p}] + \frac{D X_2}{d t_2}\bigg|_{t=0}\\
	& = -\frac{D }{d t_1}\left(\log_{(\cdot)} f_1((\cdot),\xi_n) \right)\bigg|_{t=0} + D_{\xi_n}X_1[\eta_{\xi_n}] + D_{p}X_2[\eta_{p}] + \frac{D }{d t_2} \left( (\cdot) - f_2(p,\cdot)\right)\bigg|_{t=0}.\\
	\intertext{Using the chain rule for the first term and $\frac{D }{d t_2}  (\cdot)\big|_{t=0} = I[\eta_{\xi_n}] = \eta_{\xi_n}$ for the last one we get}
	& = -\frac{D }{d t_1}\left(\log_{(\cdot)} f_1(p,\xi_n) \right)\bigg|_{t=0} - \frac{D }{d t_1}\left(\log_{p} f_1(\cdot,\xi_n) \right)\bigg|_{t=0}+ D_{\xi_n}X_1[\eta_{\xi_n}] \nonumber \\
	&  + D_{p}X_2[\eta_{p}] + \eta_{\xi_n} -\frac{D }{d t_2} \left( f_2(p,\cdot)\right)\bigg|_{t=0}\\
	& = -\nabla_{\eta_{p}}\left(\log_{(\cdot)} f_1(p,\xi_n) \right) - D_p\left(\log_{p} f_1((\cdot),\xi_n) \right)[\eta_p]+ D_{\xi_n}X_1[\eta_{\xi_n}] \nonumber \\
	& + D_{p}X_2[\eta_{p}] + \eta_{\xi_n} - \nabla_{\eta_{\xi_n}} f(p,\cdot) .
	\label{eq: cov final}
\end{align}

%the following chain rule for covariant derivatives
%\begin{equation}
%\nabla_{\xi_p} (Y \circ f)  = \nabla_{D_p f [\xi]} Y
%\end{equation}
%which follows directly from the defintion: \todo{dit slaat nergens op. Hier waarschijnlijk maar gebruiken dat we de dif van log als cov kunnen nemen}
%\begin{equation}
%\nabla_{\xi_p} (Y \circ f) = \pi^{\parallel}(\frac{d}{dt}((Y \circ f) \circ \gamma)|_{t=0}) = \pi^{\parallel}(\frac{d}{dt}(Y \circ (f \circ \gamma))|_{t=0}) = \nabla_{D_p f [\xi]} Y.
%\end{equation}
%\todo{hier laten zien dat we eigenlijk voor X1 een cov en een differential krijgen}
%Secondly, we should realize the tangent space to a product manifold is the direct sum of the tangent spaces of the basis manifolds, i.e., we may write $Y = Y_p + Y_\xi$ where $Y_p \in \mathcal{T}_p\mathcal{M}$ and $Y_\xi \in \mathcal{T}_\xi(\mathcal{T}_n\mathcal{N}) = \mathcal{T}_n\mathcal{N}$. Now we can also split the covariant derivative
%
%
%that for fixed $p$, $X_1(p,\cdot): \mathcal{T}_n \mathcal{N} \rightarrow \mathcal{T}_p \mathcal{M}$
%

For our purposes, we do not have a smooth $X$, but as for now we have only discussed generalized covariant derivatives, whereas we see from the expression above that we also need a generalization of the differential. First we need another generalization of Rademacher's theorem. The result in \cref{sec: RSSN Newton} helps us to formulate the following result.

\begin{theorem}
	Let $\mathcal{M}$ and $\mathcal{N}$ be smooth manifolds. If $F:\mathcal{M}\rightarrow \mathcal{N}$ is a locally Lipschitz continuous function, then $F$ is almost everywhere differentiable on $\mathcal{M}$.
\end{theorem}
\begin{proof}
	The proof is the same as \cite[Thm. 10]{de2018newton} only with a general manifold $\mathcal{N}$ instead of $\mathcal{T}\mathcal{M}$.
\end{proof}
The generalized differential can now be defined as follows.
\begin{definition}[Clarke generalized differential]
	The \emph{Clarke generalized differential} $D_C F$ of a locally Lipschitz continuous function $F:\mathcal{M}\rightarrow \mathcal{N}$ is the set-valued mapping defined as
	\begin{equation}
		D_{C} F(p) :=\operatorname{co}\left\{V \in \mathcal{L}\left(\mathcal{T}_{p} \mathcal{M},\mathcal{T}_{F(p)} \mathcal{N}\right): \exists\left\{p_{k}\right\} \subset \mathcal{D}_{F}, \lim _{k \rightarrow+\infty} p_{k}=p, \; V=\lim _{k \rightarrow+\infty} D_{p^k} F \right\}
	\end{equation}
	where $\mathcal{D}_{F}\subset \mathcal{M}$ is the set on which $F$ is differentiable, \enquote{co} represents the convex hull and $\mathcal{L}\left(\mathcal{T}_{p} \mathcal{M},\mathcal{T}_{F(p)} \mathcal{N}\right)$ denotes the vector space consisting of all bounded linear operator from $\mathcal{T}_{p}\mathcal{M}$ to $\mathcal{T}_{F(p)} \mathcal{N}$.
\end{definition}

Finally, the generalized covariant derivative will have the form
%\footnote{Note that $X^2$ lives in a vector space so the generalized covariant derivative reduces to the generalized differential as discussed in chapter 3.}
\begin{equation}
	\partial_{\mathcal{M},C} X(p,\xi_n) = \begin{bmatrix}
		\partial_{\mathcal{M},C,p} X_1 & D_{C,\xi_n} X_1 \\ 
		D_{C,p} X_2 & \partial_{C,\xi_n} X_2
	\end{bmatrix} ,
\end{equation}
where 
\begin{align}
	\partial_{\mathcal{M},C,p} X_1 &= -\partial_{C,\mathcal{M},p}\left(\log_{(\cdot)} f_1(p,\xi_n) \right) - D_{C,p}\left(\log_{p} f_1((\cdot),\xi_n) \right),\\
	\partial_{C,\xi_n} X_2 &= I - \partial_{C,\xi_n} f(p,\cdot).
\end{align}

Actually computing the generalized covariant derivative \cref{eq: Newton}\todo{new label} for a general manifold can be complicated. In this work we will focus on symmetric manifolds as discussed in \cref{sec: Riemannian geometry}. In \cref{sec: Jacobi fields} we saw that for symmetric manifolds we know the differentials and/or covariant derivatives of geodesics, exponential and logarithmic maps. If we also use that in symmetric spaces the parallel transport map is exactly the pole ladder \cite{pennec2018parallel} - which is also formulated in terms of logarithmic, exponential and geodesic maps - we have exact expressions for the full generalized covariant derivative, with the exception of the differentials of the proximal maps. As we shall see in \cref{sec: RSSN application}, for $\ell^2$-TV we even have exact expressions for the proxes on top of that.

==> sections/A-Numerics.tex <==
\section{Numerics}
\label{app: numerics}

\paragraph{Proximal Maps and Generalized Differentials}

\todo{Ronny: 3) For Jacobi fields, great to see them in action, Johannes Persch collected most the the Jacobi fields in his thesis, some can also be found in the TGV paper I think (S0898122118302062) or in the Paper with Pierre-Yves (full) that’s at least how I got to implement them and why I am urging my Manifolds.jl codevelops to provide ONBs with curvature eigenvalues .}
Then we have for the data fidelity term \cite[Prop. 4.4]{bergmann2018recent}
\begin{align}
	\operatorname{prox}_{\sigma F}(p) = \gamma_{p,h} \left(\frac{\sigma}{\alpha + \sigma}\right)
\end{align}
and we find
\begin{equation}
	D_{C,p} \operatorname{prox}_{\sigma F}(p) = D_p \operatorname{prox}_{\sigma F}(\cdot) = D_p \gamma_{(\cdot),h} \left(\frac{\sigma}{\alpha + \sigma}\right),
\end{equation}
where we used that $\operatorname{prox}_{\sigma F}(x)$ is smooth. Hence, we can choose $B = D_p \gamma_{(\cdot),h} \left(\frac{\sigma}{\alpha + \sigma}\right)$ for the Newton operator.

For the dual variable we live in a vector space. The proximal mapping comes down to the same as we have already computed in \cref{sec: Newton application}, but with a modification for the point part, i.e, for $\xi_n = (\xi_m^1, \xi_m^2) \in \mathcal{T}_m^* \mathcal{M}^{d_1\times d_2 \times 2} \times \mathcal{T}_m^* \mathcal{M}^{d_1\times d_2 \times 2}$
\begin{equation} 
	\operatorname{prox}_{\tau G^*_{n,1}}(\xi_{n}) = \left(0, \left(\max \left\{1,\|(\xi_{m}^2)_{i, j, k} \|_m\right\}\right)^{-1} (\xi_{m}^2)_{i, j, k}\right)_{i, j, k} 
\end{equation}
and
\begin{equation}
	\operatorname{prox}_{\tau G^*_{n,2}}(\xi_n) = \left(0,\left(\max \left\{1, \|  (\xi_{m}^2)_{i,j,:} \|_{m,2} \right\}\right)^{-1} (\xi_{m}^2)_{i, j, k}\right)_{i, j, k}.
\end{equation}

Since the point part is always mapped to $0$, this will be incorporated into the optimality system right away in order to reduce the matrix dimentions. For the optimality system we write
\begin{align}
	p &= \operatorname{prox}_{\sigma F}\left(\exp _{p}\left(\mathcal{P}_{m\rightarrow p} \left(-\sigma \left(D_m \Lambda\right)^{*}\left[ \xi_{m}\right]\right)^{\sharp}\right)\right), \\
	\xi_{n} &= \operatorname{prox}_{\tau G_{m}^{*}}\left(\xi_{m}+\tau\left(\mathcal{P}_{\Lambda\left(m\right) \rightarrow n} D_m \Lambda\left[\log _{m} p\right]\right)^{\flat}\right).
\end{align}

Then, the generalized covariant derivative applied to $\eta_n = (\eta_m^1, \eta_m^2)$ is given by


\begin{equation}
	(J_1(\xi_n) \eta_n)_{i, j, k}=\left\{\begin{array}{ll}
		(0,0)  & \text { if } i=d_{1} \text { and } k=1 \\
		(0,0)  & \text { if } j=d_{2} \text { and } k=2 \\
		(0,(\eta_m^2)_{i,j,k})  & \text { if } \|(\xi_m^2)_{i,j,:}\|_{m} \leq 1 \\
		\left(0, \frac{1}{\| (\xi_m^2)_{i,j,k} \|_{m}}\left( (\eta_m^2)_{i,j,k} -  \frac{\langle (\xi_m^2)_{i,j,k}, (\eta_m^2)_{i,j,k} \rangle_m}{\| (\xi_m^2)_{i,j,k} \|_{m}^2}(\xi_m^2)_{i,j,k} \right) \right) & \text { if } \|(\xi_m^2)_{i,j,k}\|_{m} > 1
	\end{array}\right.
\end{equation}
and
\begin{equation}
	(J_2(\xi_n) \eta_n)_{i, j, k}=\left\{\begin{array}{ll}
		(0,0)  & \text { if } i=d_{1} \text { and } k=1 \\
		(0,0)  & \text { if } j=d_{2} \text { and } k=2 \\
		(0,(\eta_m^2)_{i,j,k})  & \text { if } \|(\xi_m^2)_{i,j,:}\|_{m,2} \leq 1 \\
		\left(0,\frac{1}{\| (\xi_m^2)_{i,j,:} \|_{m,2}}\left( (\eta_m^2)_{i,j,k} - \sum_{\kappa=1,2} \frac{\langle (\xi_m^2)_{i,j,\kappa}, (\eta_m^2)_{i,j,\kappa} \rangle_m}{\| (\xi_m^2)_{i,j,:} \|_{m,2}^2}(\xi_m^2)_{i,j,k} \right)  \right) & \text { if } \|(\xi_m^2)_{i,j,:}\|_{m,2} > 1
	\end{array}\right.
\end{equation}
where the operator $J_1$ corresponds to anisotropic TV and $J_2$ to isotropic. Here the first two conditions ensure the boundary conditions $y_{i,j,k} = 0$ for $i=d_{1} \text { and } k=1$ or  $j=d_{2} \text { and } k=2$. The third and fourth options should be understood as the case of not being a boundary point, i.e., $i<d_{1} \text { and } k=1 $ and $j<d_{2} \text { and } k=2$. A proof can be found in \cref{sec: app2}.

For the semismoothness we already have that $\operatorname{prox}_{\sigma F}(x)$ is semismooth since it is smooth: by the generalized Taylor series in \cite{dedieu2003newton} we find semismoothness according to \cref{def: semismooth manifold}. The semismoothness of $\operatorname{prox}_{\tau G^*_q}(y)$ follows from invoking \cref{prop: C1 semismooth} as in the non-manifold case. Indeed we can do this, since the dual variable just lives in a finite dimensional vector space, which is isomorphic with $\mathbb{R}^d$. So we are indeed justified to use RSSN for $\ell^2$-TV.

\begin{remark}
	As we see from the formulation of the optimization problem to computing the dual proximal maps, the point part does not play an important role in the optimization problem: it is always zero. Therefore we can focus solely on the vector part in the following. To start of, we can ignore the point part for the proximal map in implementations and also drop them for computing $J$. This gives as an extra advantage that the Newton matrix becomes smaller. 
\end{remark}

\paragraph{Linearization of the Operator $T$}
Next, to derive $D_m T$ and its adjoint, let $p \in \mathcal{M}^{d_{1} \times d_{2}}$ and $v \in \mathcal{T}_{p} \mathcal{M}^{d_{1} \times d_{2}}$. We follow the approach in \cite[Sect. 5]{bergmann2019fenchel}. First, applying the chain rule we find 
\begin{equation}
	(D_p T[v])_{i, j, k} = D_{p_{i,j}} \log _{(\cdot)}\left(p_{i, j+e_{k}}\right)\left[v_{i, j}\right]+D_{p_{i, j+e_{k}}} \log _{p_{i, j}}(\cdot)\left[v_{i, j+e_{k}}\right],
	\label{eq: DT}
\end{equation}
with the obvious modifications at the boundary. In the above formula $e_{k}$ represents either the vector (0,1) or (1,0) used to reach either the neighbour to the right $(k=1)$ or below $(k=2)$. 

Again, we use the decomposition of the tangent bundle tangent space. As noted in the previous remark, the point part does not bring new information. Using the result in \cref{eq: log diff}, \cref{eq: DT} reduces to
\begin{equation}
	(D_p T[v])_{i, j, k}^v = \nabla_{v_{p_{i, j}}} \log _{(\cdot)}\left(p_{i, j+e_{k}}\right) + D_{p_{i, j+e_{k}}} \log _{p_{i, j}}(\cdot)\left[v_{i, j+e_{k}}\right] \in \mathcal{T}_{p_{i,j}} \mathcal{M},
	\label{eq: DT 2}
\end{equation}
where the superscript $v$ denotes the vector part of the tangent space. We used that that the second term only gave a contribution to the vector part of the tangent bundle tangent space in the first place.  We can compute these maps using Jacobi fields as discussed in \cref{prop: jacobi fields}. With a slight abuse of notation we will drop the superscript $v$ in the following since we know that we only use the vector part of the tangent space. Then, we have\footnote{Here the decomposition originates from the two components represented by $k=1$ and $k =2$. This should not be confused with the point and vector part of the tangent space of the tangent bundle.} $(D_p T): \mathcal{T}_p \mathcal{M}^{d_{1} \times d_{2}} \rightarrow \mathcal{T}_{p} \mathcal{M}^{d_{1} \times d_{2}\times 2} (= \mathcal{T}_p \mathcal{M}^{d_{1} \times d_{2}}\times \mathcal{T}_p \mathcal{M}^{d_{1} \times d_{2}})$ given by Jacobi fields. 

Subsequently, its adjoint can be computed using the adjoint Jacobi fields as given in \cref{eq: adjoint jacobi}. Following the same line of reasoning, note that we should also focus on the vector part of the dual space, i.e., $\mathcal{T}_{p}^* \mathcal{M}^{d_{1} \times d_{2}\times 2}$ instead of looking at the entire space $\mathcal{T}_{T(p)}^{*} \mathcal{T}\mathcal{M}^{d_1\times d_2\times 2}$. Define $N_{i, j}$ to be the set of neighbours of the pixel $p_{i, j}$ and let $\eta \in \mathcal{T}_{(p,p)}^* \mathcal{M}^{d_{1} \times d_{2}\times 2}$ then we can find \cite[Sect. 5]{bergmann2019fenchel}
\begin{equation}
	\left(D_p T[\eta]\right)_{i, j}^{*}=\sum_{k} \left(\nabla \log _{(\cdot)}\left(p_{i, j+e_{k}}\right)\right)^*\left[\eta_{i, j, k}\right] \; +\sum_{\left(i^{\prime}, j^{\prime}\right) \in N_{i, j}} \left(D_{p_{i,j}} \log _{p_{i',j'}} (\cdot) \right)^*\left[\eta_{i^{\prime} j^{\prime} k}\right].
\end{equation}

\paragraph{Regularization of the Dual} 
In the case of $\mathbb{R}^n$ we saw in \cref{sec: loops} that the Newton matrix became non-invertible. For general manifolds we are now motivated to look to the dual regularized $\ell^2$-TV saddle-point problem
\begin{equation}
	\inf_{p \in \mathcal{M}^{d_1\times d_2}} \sup_{\xi_{n} \in \mathcal{T}_{n}^* \mathcal{T}\mathcal{M}^{d_1\times d_2\times 2}}  \frac{1}{2 \alpha} \sum_{i, j=1}^{d_{1}, d_{2}} d_{\mathcal{M}}^{2}\left(p_{i, j},h_{i, j}\right) + \langle \log_n T(p) ,\xi_n \rangle_n - \iota_{\{0\}\times B_{q^*}}(\xi_n) - \frac{\beta}{2}\|\xi_n\|_n^2
\end{equation}
and hence consider $\tilde{G}^*_{n,1} = \iota_{\{0\}\times B_{q^*}}(\xi_n) + \frac{\beta}{2}\|\xi_n\|_n^2$. Then, as with the linear case it is not hard to see that the proximal maps become
\begin{equation} 
	\operatorname{prox}_{\tau \tilde{G}^*_{n,1}}(\xi_{n}) = \left(0,\left(\max \left\{1,\frac{\|(\xi_{m}^2)_{i, j, k} \|_m}{1 + \beta \tau}\right\}\right)^{-1} \frac{(\xi_{m}^2)_{i, j, k}}{1 + \beta \tau}\right)_{i, j, k} 
\end{equation}
and
\begin{equation}
	\operatorname{prox}_{\tau \tilde{G}^*_{n,2}}(\xi_n) = \left(0,\left(\max \left\{1, \frac{\|  (\xi_{m}^2)_{i,j,:} \|_{m,2}}{1 + \beta \tau} \right\}\right)^{-1} \frac{(\xi_{m}^2)_{i, j, k}}{1 + \beta \tau}\right)_{i, j, k}
\end{equation}
and as with the regular proxes we find for the covariant derivatives
\begin{equation}
	(J_1(\xi_n) \eta_n)_{i, j, k}=\left\{\begin{array}{ll}
		(0,0)  & \text { if } i=d_{1} \text { and } k=1 \\
		(0,0)  & \text { if } j=d_{2} \text { and } k=2 \\
		(0,(\eta_m^2)_{i,j,k})  & \text { if } \|(\xi_m^2)_{i,j,:}\|_{m} \leq 1 + \beta \tau \\
		\left(0, \frac{1}{\| (\xi_m^2)_{i,j,k} \|_{m}}\left( (\eta_m^2)_{i,j,k} -  \frac{\langle (\xi_m^2)_{i,j,k}, (\eta_m^2)_{i,j,k} \rangle_m}{\| (\xi_m^2)_{i,j,k} \|_{m}^2}(\xi_m^2)_{i,j,k} \right) \right) & \text { if } \|(\xi_m^2)_{i,j,k}\|_{m} > 1 + \beta \tau
	\end{array}\right.
\end{equation}
and
\begin{equation}
	(J_2(\xi_n) \eta_n)_{i, j, k}=\left\{\begin{array}{ll}
		(0,0)  & \text { if } i=d_{1} \text { and } k=1 \\
		(0,0)  & \text { if } j=d_{2} \text { and } k=2 \\
		(0,(\eta_m^2)_{i,j,k})  & \text { if } \|(\xi_m^2)_{i,j,:}\|_{m,2} \leq 1 + \beta \tau \\
		\left(0,\frac{1}{\| (\xi_m^2)_{i,j,:} \|_{m,2}}\left( (\eta_m^2)_{i,j,k} - \sum_{\kappa=1,2} \frac{\langle (\xi_m^2)_{i,j,\kappa}, (\eta_m^2)_{i,j,\kappa} \rangle_m}{\| (\xi_m^2)_{i,j,:} \|_{m,2}^2}(\xi_m^2)_{i,j,k} \right)  \right) & \text { if } \|(\xi_m^2)_{i,j,:}\|_{m,2} > 1 + \beta \tau
	\end{array}\right.
\end{equation}


\begin{remark}
	For a general manifold we did not show that we run into ill-posedness issues. However, from numerical observations it seems to be the case for 2D problems (as in the $\mathbb{R}^n$ case). Actually showing this remains an open problem. 
\end{remark}
